Feature emergence via margin maximization: case studies in algebraic tasks

Understanding the internal representations learned by neural networks is a cornerstone challenge in the science of machine learning. While there have been significant recent strides in some cases towards understanding how neural networks implement specific target functions, this paper explores a complementary question -- why do networks arrive at particular computational strategies? Our inquiry focuses on the algebraic learning tasks of modular addition, sparse parities, and finite group operations. Our primary theoretical findings analytically characterize the features learned by stylized neural networks for these algebraic tasks. Notably, our main technique demonstrates how the principle of margin maximization alone can be used to fully specify the features learned by the network. Specifically, we prove that the trained networks utilize Fourier features to perform modular addition and employ features corresponding to irreducible group-theoretic representations to perform compositions in general groups, aligning closely with the empirical observations of Nanda et al. and Chughtai et al. More generally, we hope our techniques can help to foster a deeper understanding of why neural networks adopt specific computational strategies.

==> backbone-theorem.tex <==
\newcommand{\lnorm}[2]{\Vert #1 \Vert_{#2}}
\newcommand{\ltwonorm}[1]{\lnorm{#1}{2}}
\renewcommand{\P}{\mathop{\mathbb{P}}}
\newcommand{\integers}{\mathbb{Z}}
\newcommand{\fhat}{\widehat{f}}
\newcommand{\curlyg}{\mathcal{G}}
\newcommand{\curlym}{\mathcal{M}}
\newcommand{\normal}{\mathcal{N}}
\newcommand{\curlyf}{\mathcal{F}}
\newcommand{\curlyx}{\mathcal{X}}
\newcommand{\curlyy}{\mathcal{Y}}
\newcommand{\curlyh}{\mathcal{H}}
\newcommand{\curlyp}{\mathcal{P}}
\newcommand{\estoff}{\mathsf{Est_{Sq}^{off}}}
\newcommand{\spt}{\mathrm{spt}}
\newcommand{\expct}{\mathop{{}\mathbb{E}}}
\renewcommand{\CO}[1]{\textcolor{orange}{(\textbf{Costin:} #1)}}

% \newcommand{\vx}{\mathbf{x}}
% \newcommand{\vw}{\mathbf{w}}
% \newcommand{\sign}{\mathrm{sign}}
% 
% \newcommand{\ve}{\mathbf{e}}
% \newcommand{\vzero}{\mathbf{0}}
% \newcommand{\vv}{\mathbf{v}}
% \newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
% \newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
% \newcommand{\argmin}{\mathop{\mathrm{argmin}}
% \newcommand{\argmax}{\mathop{\mathrm{argmax}}

\newpage
\section{General Theorem}
Suppose we have a dataset $D \subseteq \curlyx \times \curlyy$, a class of parameterized functions $\{\Phi(\theta, \cdot) \mid \theta \in \Theta\}$, where $\Phi : \Theta \times \curlyx \to \R ^ \curlyy$ and a distribution $\nu$ over the compact parameter space $\Theta$ which induces the function $f : \curlyp(\Theta) \times \curlyx \to \R ^ \curlyy$ given by $f(\nu, x) = \int_{\theta \in \Theta} \Phi(\theta, x)d\nu(\theta)$.
We define the margin function $g : \curlyp(\Theta) \times \curlyx \times \curlyy \to \R$ as being, for a given datapoint $(x, y) \in D$, $g(\nu, x, y) = f(\nu, x)[y] - \max\limits_{y' \in \curlyy \setminus \{y\}}{f(\nu, x)[y']}$.
Then, the margin of the dataset $D$ is given by $h : \curlyp(\Theta) \to \R$ defined as $h(\nu) = \min\limits_{(x, y) \in D} g(\nu, x, y)$.
We are concerned with characterizing $\argmax \limits_{\nu \in \curlyp(\Theta)}{h(\nu)}$. \BE{Should specify that $\Theta$ is compact.}
Finally, define a helping function $g' : \curlyp(\Theta) \times \curlyx \times \curlyy \to \R$ as $g'(\nu, x, y) = f(\nu, x)[y] - \frac{1}{|\curlyy|-1}\sum\limits_{y' \in \curlyy \setminus \{y\}}{f(\nu, x)[y']}$ for any given datapoint $(x, y) \in D$. Note that the difference between $g'$ and $g$ is using mean instead of $\max$ of the outputs at all incorrect labels. Hence, one direct consequence is that $g'(\nu, x, y) \geq g(\nu, x, y)$ with equality when all outputs at positions other than $y$ are equal.

% The crux of Theorem~\ref{backbone-theorem} is that

Suppose we have two distributions $\nu^* \in \curlyp(\Theta)$ over parameterizations of $\Phi$ and $p^* \in \curlyp(D)$ over datapoints in $D$ and consider the following conditions on these:

\begin{enumerate}[label=\textbf{C.\arabic*}]
    \item \label{c1} $p^* \in \argmin\limits_{p \in \curlyp(D)}{\sum\limits_{(x, y) \in D}{p((x, y))g(\nu^*, x, y)}}$. Equivalently, $\spt(p^*) \subseteq \argmin\limits_{(x,y) \in D}{g(\nu^*, x, y)}$.
    \item \label{c2} $\nu^* \in \argmax\limits_{\nu \in \curlyp(\Theta)}{\sum\limits_{(x, y) \in D}{p^*((x, y))g(\nu, x, y)}}$
    \item \label{c3} for any $(x, y) \in D$, it holds that $g'(\nu^*, x, y) = g(\nu^*, x, y)$. This is equivalent to saying that for any $y', y'' \in \curlyy \setminus \{y\}$, we have $f(\nu^*, x)[y'] = f(\nu^*, x)[y'']$.
    \item \label{c4} $\nu^* \in \argmax\limits_{\nu \in \curlyp(\Theta)}{\sum\limits_{(x, y) \in D}{p^*((x, y))g'(\nu, x, y)}}$
\end{enumerate}
Here and henceforth, we let $\spt(p) := \{(x, y) : p(x,y) > 0\}$.

% We start with a lemma that says that \ref{c3} allows for a change from $g'$ to $g$ in \ref{c2}.
\begin{lemma}
\label{c34implies2}
Suppose conditions \ref{c3} and \ref{c4} hold. Then \ref{c2} also holds and $\argmax\limits_{\nu \in \curlyp(\Theta)}{\sum\limits_{(x, y) \in D}{p^*((x, y))g(\nu, x, y)}} \subseteq \argmax\limits_{\nu \in \curlyp(\Theta)}{\sum\limits_{(x, y) \in D}{p^*((x, y))g'(\nu, x, y)}}$.
\end{lemma}
\begin{proof}
\begin{align*}
& \max\limits_{\nu \in \curlyp(\Theta)}{\sum\limits_{(x, y) \in D}{p^*((x, y))g(\nu, x, y)}} \leq
\max\limits_{\nu \in \curlyp(\Theta)}{\sum\limits_{(x, y) \in D}{p^*((x, y))g'(\nu, x, y)}} = \sum\limits_{(x, y) \in D}{p^*((x, y))g'(\nu^*, x, y)} = \\
& \sum\limits_{(x, y) \in D}{p^*((x, y))g(\nu^*, x, y)} \leq \max\limits_{\nu \in \curlyp(\Theta)}{\sum\limits_{(x, y) \in D}{p^*((x, y))g(\nu, x, y)}}
\end{align*}
where the first equality follow from \ref{c4} and the second follows from \ref{c3}. Since we bound all terms between two equal values, the inequalities are in fact equalities and the first part of the statement follows. For the second, take some $\nu^{**} \in \argmax\limits_{\nu \in \curlyp(\Theta)}{\sum\limits_{(x, y) \in D}{p^*((x, y))g(\nu, x, y)}}$. By previous equalities, it follows that:
\begin{align*}
    \max\limits_{\nu \in \curlyp(\Theta)}{\sum\limits_{(x, y) \in D}{p^*((x, y))g'(\nu, x, y)}} = \sum\limits_{(x, y) \in D}{p^*((x, y))g(\nu^{**}, x, y)} \leq \sum\limits_{(x, y) \in D}{p^*((x, y))g'(\nu^{**}, x, y)}
\end{align*}
Hence, $\nu^{**} \in \argmax\limits_{\nu \in \curlyp(\Theta)}{\sum\limits_{(x, y) \in D}{p^*((x, y))g'(\nu, x, y)}}$, which concludes the proof.
\end{proof}

\begin{lemma}
\label{c12impliesall}
If \ref{c1} and \ref{c2} hold then it holds that $\nu^* \in \argmax \limits_{\nu \in \curlyp(\Theta)}{h(\nu)}$.
\end{lemma}
\begin{proof}
First, by rewriting the definition of $h$ and using weak duality, we have:
\begin{align*}
    & \max\limits_{\nu \in \curlyp(\Theta)}{h(\nu)} = \max\limits_{\nu \in \curlyp(\Theta)}{\min\limits_{(x, y) \in D}{g(\nu, x, y)}} = \max\limits_{\nu \in \curlyp(\Theta)}\min\limits_{p \in \curlyp(D)}{\sum\limits_{(x, y) \in D} p((x, y))g(\nu, x, y)} \leq \\
    & \min\limits_{p \in \curlyp(D)}\max\limits_{\nu \in \curlyp(\Theta)}{\sum\limits_{(x, y) \in D} p((x, y))g(\nu, x, y)}
\end{align*}
On the other hand, it also holds that:
\begin{align*}
    & \min\limits_{p \in \curlyp(D)}\max\limits_{\nu \in \curlyp(\Theta)}{\sum\limits_{(x, y) \in D} p((x, y))g(\nu, x, y)} \leq 
    \max\limits_{\nu \in \curlyp(\Theta)}{\sum\limits_{(x, y) \in D} p^*((x, y))g(\nu, x, y)} = \\
    & \sum\limits_{(x, y) \in D} p^*((x, y))g(\nu^*, x, y) = \min\limits_{p \in \curlyp(D)}{\sum\limits_{(x, y) \in D} p((x, y))g(\nu^*, x, y)} \leq \\
    & \max\limits_{\nu \in \curlyp(\Theta)}\min\limits_{p \in \curlyp(D)}{\sum\limits_{(x, y) \in D} p((x, y))g(\nu, x, y)}
\end{align*}
where the first equality follows from \ref{c2} and the second follows from \ref{c1}. Putting these inequalities together it follows that all of the above terms are equal (and, thus, strong duality holds). In particular, $\max\limits_{\nu \in \curlyp(\Theta)}{h(\nu)} = \min\limits_{p \in \curlyp(D)}{\sum\limits_{(x, y) \in D} p((x, y))g(\nu^*, x, y)} = h(\nu^*)$ as desired.
\end{proof}

\begin{theorem}
\label{backbone-theorem}
If \ref{c1}, \ref{c3} and \ref{c4} hold, then it holds that $\nu^* \in \argmax \limits_{\nu \in \curlyp(\Theta)}{h(\nu)}$. Furthermore, if $\spt(p^*) = D$, it follows that $\argmax \limits_{\nu \in \curlyp(\Theta)}{h(\nu)} \subseteq \argmax\limits_{\nu \in \curlyp(\Theta)}{\sum\limits_{(x, y) \in D}{p^*((x, y))g'(\nu, x, y)}}$.
\end{theorem}
\begin{proof}
By Lemma \ref{c34implies2} it follows that \ref{c2} holds. Consequently, we can apply Lemma \ref{c12impliesall} to get the first part of the statement.

For the second part, suppose $\spt(p^*)=D$ and let $\gamma = \max \limits_{\nu \in \curlyp(\Theta)}{h(\nu)} = h(\nu^*)$.
% By \ref{c1}, it follows that the margin induced by $\nu^*$ is the same for all datapoints in $D$, namely, for any $(x, y) \in D$, we have $g(\nu^*, x, y)=\gamma$.
Let $\nu^{**} \in \argmax \limits_{\nu \in \curlyp(\Theta)}{h(\nu)}$. Hence, $\gamma = h(\nu^{**}) = \min\limits_{(x, y) \in D} g(\nu^{**}, x, y)$.

If there existed any $(x, y) \in D$ such that $g(\nu^{**}, x, y)>\gamma$, by $p^*((x, y)) > 0$, it would follow that $\sum\limits_{(x, y) \in D}{p^*((x, y))g(\nu^{**}, x, y)} > \gamma = \sum\limits_{(x, y) \in D}{p^*((x, y))g(\nu^*, x, y)}$.
However, this contradicts \ref{c2}, so it must be that $g(\nu^{**}, x, y)=\gamma$ for all $(x, y) \in D$.
Thus, $\sum\limits_{(x, y) \in D}{p^*((x, y))g(\nu^{**}, x, y)} = \gamma = \sum\limits_{(x, y) \in D}{p^*((x, y))g(\nu^*, x, y)} = \max\limits_{\nu \in \curlyp(\Theta)}{\sum\limits_{(x, y) \in D}{p^*((x, y))g(\nu, x, y)}}$ where the last equality follows from \ref{c2}.
Hence, $\nu^{**} \in \argmax\limits_{\nu \in \curlyp(\Theta)}{\sum\limits_{(x, y) \in D}{p^*((x, y))g(\nu, x, y)}}$. Combining this with second part of Lemma~\ref{c34implies2}, the conclusion follows.

% \item Or there exists some $(x, y) \in D$ such that $g(\nu^{**}, x, y)>\gamma$. But then, since $p^*((x, y)) > 0$, it follows that $\sum\limits_{(x, y) \in D}{p^*((x, y))g(\nu^{**}, x, y)} > \gamma = \sum\limits_{(x, y) \in D}{p^*((x, y))g(\nu^*, x, y)}$. However, this contradicts \ref{c2}.

\end{proof}

\subsection{Neural network as parameterized functions}
Consider a single neuron in a two layer neural network given by
\[ \phi(u, b, w; x) = w \sigma(u^\top x + b)\]
where $u$ and $w$ are the first and second layer weights of the neuron respectively, $b$ is the bias of the first layer and $\sigma$ represents the activation function. A neural network of width $m$ is given by 
\[ f(\{u_i, b_i, w_i\}_{i=1}^m; x) = \sum_{i=1}^m \phi(u_i, b_i, w_i; x) \]
As we are considering $\sigma$ to be the quadratic activation, i.e, $\sigma(x) = x^2$, by two homogeneity of the activation, we can say
\[ f(\{u_i, b_i, w_i\}_{i=1}^m; x) = \sum_{i=1}^m \| u_i, b_i, w_i \|^3 \phi\left(\frac{u_i}{\| u_i, b_i, w_i \|}, \frac{b_i}{\| u_i, b_i, w_i \|}, \frac{w_i}{\| u_i, b_i, w_i \|}; x\right) \]
where $\| u_i, b_i, w_i \|$ represents the norm of the concatentation of $u_i, b_i$ and $w_i$. Denoting $(u_i, b_i, w_i)$ as $\theta_i$, we can say
\[ f(\{\theta_i\}_{i=1}^m; x) = \sum_{i=1}^m \| \theta_i \|^3 \phi\left(\frac{\theta_i}{\| \theta_i \|}; x\right) \]
Thus, the neural network can be thought of as operating on the direction $\theta_i$, with a mass of $\| \theta_i \|^3$. Thus, a natural way to regularize the output of this network is to bound its total mass on the unit norm sphere given by $\sum_{i=1}^m \|\theta_i\|^3$. 

% \CO{I could also put the lemma and the theorem together directly but since there are a bunch of constrain}
